Understanding Inter-Concept Relationships in Concept-Based Models

Concept-based explainability methods provide insight into deep learning systems by constructing explanations using human-understandable concepts. While the literature on human reasoning demonstrates that we exploit relationships between concepts when solving tasks, it is unclear whether concept-based methods incorporate the rich structure of inter-concept relationships. We analyse the concept representations learnt by concept-based models to understand whether these models correctly capture inter-concept relationships. First, we empirically demonstrate that state-of-the-art concept-based models produce representations that lack stability and robustness, and such methods fail to capture inter-concept relationships. Then, we develop a novel algorithm which leverages inter-concept relationships to improve concept intervention accuracy, demonstrating how correctly capturing inter-concept relationships can improve downstream tasks.

==> sections/rebuttal.tex <==
\begin{figure*}
    \centering
    \subfloat[\centering CUB]{\includegraphics[width=0.3 \textwidth]{figures/cub_intervention.pdf}}
    \subfloat[\centering Coloured MNIST]{\includegraphics[width=0.3 \textwidth]{figures/mnist_intervention.pdf}}
    \subfloat[\centering dSprites]{\includegraphics[width=0.3 \textwidth]{figures/dsprites_intervention.pdf}}  
    \caption{
        On the CUB and MNIST datasets, label bases improve concept intervention accuracy when compared with interventions made without concept bases or using other concept bases. Additionally, poorly constructed concept bases (TCAV, CEM) hurt accuracy by up to $10\%$ in CUB. 
        % We vary the fraction of concept groups intervened upon and see that Shapley and Label vectors consistently lead to higher accuracy on concept intervention. Compared to not using a concept basis, using a concept basis has the biggest impact when intervening between 20\% and 80\% of concepts. When using other concept-based methods, such as TCAV and CEM, we see that the concept intervention performance is near or worse than the baseline.
    }
        \label{fig:intervention_dataset}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/ois_scores.pdf}
    \caption{CEM bases have larger (worse) oracle impurity scores than label bases across datasets, indicating that they are more impure representations of the underlying concepts.}
    \label{fig:ois_score}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/ois_scatter.pdf}
    \caption{We compare OIS and robustness for the CEM and Label bases and find that across most datasets, more robust representations correspond to better (lower) oracle impurity scores (OIS). This shows that the robustness metric captures the quality of the representation itself.  }
    \label{fig:ois_scatter}
\end{figure}

\begin{figure}
    \centering
    \subfloat[\centering Concept Acc.]{\includegraphics[width=0.25 \textwidth]{figures/concept_correlations_mnist_c.pdf}}
    \subfloat[\centering Label Acc.]{\includegraphics[width=0.25 \textwidth]{figures/concept_correlations_mnist_y.pdf}}

    \caption{Increasing correlations between concepts lead to higher accuracy for CEM models trained on the coloured MNIST dataset. We increase the correlation between the number and colour concepts from $0\%$ to $100\%$, with the correlation rate denoting the frequency at which number and colour concepts align. }
    \label{fig:ois_scatter}
\end{figure}

Sect
